In Memoriam: Peter Higgs (1929-2024)

Peter Higgs was a British theoretical physicist, famous for his work published in 1964, where he proposed a mechanism that can generate masses for elementary particles, while respecting gauge invariance. Half a century later, two experiments at CERN confirmed that this mechanism is realized in nature. On April 8th, we received the sad news of the passing of the great pioneer of elementary particle physics. This article is dedicated to his memory, and to the mechanism and particle that bear his name. -- Peter Higgs fue un f\'isico te\'orico brit\'anico, famoso por su trabajo de 1964 donde propuso un mecanismo que puede generar masas para part\'iculas elementales, conforme a la simetr\'ia de norma. Medio siglo m\'as tarde, dos experimentos del CERN confirmaron que este mecanismo est\'a realizado en la naturaleza. El 8 de abril nos lleg\'o la triste noticia del fallecimiento del gran pionero de la fisica de part\'iculas elementales. Este art\'iculo es dedicado a su memoria, as\'i como al mecanismo y a la part\'icula que llevan su nombre.

==> abs_eng.tex <==
Peter Higgs was a British theoretical physicist, famous for his work
published in 1964, where he proposed a mechanism that can generate masses
for elementary particles, while respecting gauge invariance. Half a century
later, two experiments at CERN confirmed that this mechanism is
realized in nature. On April 8th, we received the sad news of the
passing of the great pioneer of elementary particle physics. This
article is dedicated to his memory, and to the mechanism and particle
that bear his name.


==> refs_eng.tex <==
\begin{thebibliography}{10}

\bibitem{Higgs} P.W.\ Higgs,
Broken symmetries, massless particles and gauge fields,
\href{https://dx.doi.org/10.1016/0031-9163(64)91136-9}
     {{\em Phys.\ Lett.}\ {\bf 12} (1964) 132-133};
Broken Symmetries and the Masses of Gauge Bosons,
\href{https://dx.doi.org/10.1103/PhysRevLett.13.508}
     {{\em Phys.\ Rev.\ Lett.}\ {\bf 13} (1964) 508-509};
Spontaneous Symmetry Breakdown without Massless Bosons,
\href{https://dx.doi.org/10.1103/PhysRev.145.1156}
     {{\em Phys.\ Rev.}\ {\bf 145} (1966) 1156-1163}.

\bibitem{boson} P.\ Higgs,
My Life as a Boson: The Story of ``The Higgs'',
\href{https://dx.doi.org/10.1142/S0217751X02013046}
     {{\em Int.\ J.\ Phys.}\ {\bf A17} (2002) 86-88}.

\bibitem{EB} F.\ Englert and R.\ Brout,
Broken Symmetry and the Mass of Gauge Vector Mesons,
\href{https://dx.doi.org/10.1103/PhysRevLett.13.321}
     {{\em Phys.\ Rev.\ Lett.}\ {\bf 13} (1964) 321-323}.

\bibitem{GHK} G.S.\ Guralnik, C.R.\ Hagen and T.W.B.\ Kibble,
Global Conservation Laws and Massless Particles,
\href{https://dx.doi.org/10.1103/PhysRevLett.13.585}
     {{\em Phys.\ Rev.\ Lett.}\ {\bf 13} (1964) 585-587}.

\bibitem{Anderson} P.W.\ Anderson,
Plasmons, Gauge Invariance, and Mass,
\href{https://dx.doi.org/10.1103/PhysRev.130.439}
     {{\it Phys.\ Rev.}\ {\bf 130} (1963) 439-442.}

\bibitem{Schwinger} J.S.\ Schwinger,
Gauge Invariance and Mass,
\href{https://dx.doi.org/10.1103/PhysRev.125.397}
     {{\em Phys.\ Rev.}\ {\bf 125} (1962) 397-398};
Gauge Invariance and Mass. 2.,
\href{https://dx.doi.org/10.1103/PhysRev.128.2425}
     {{\em Phys.\ Rev.}\ {\bf 128} (1962) 2425-2429}.

\bibitem{Nobel13} Royal Swedish Academy of Sciences,
  \href{https:www.nobelprize.org/prizes/physics/2013/advanced-information}
       {Scientific Background: The BEH-Mechanism, Interactions with Short
  Range Forces and Scalar Particles}
  
\bibitem{MigPol} A.A.\ Migdal and A.M.\ Polyakov,
Spontaneous breakdown of strong interaction symmetry
and the absence of massless particles,
{\em Zh.\ Eksp.\ Teor.\ Fiz.}\ {\bf 51} (1966) 135-146 
[\href{http://www.jetp.ras.ru/cgi-bin/dn/e_024_01_0091.pdf}
  {{\em Sov.\ Phys.\ JETP} {\bf 24} (1967) 91-98}].

\bibitem{Weinberg} S.\ Weinberg,
A Model of Leptons,
\href{https://dx.doi.org/10.1103/PhysRevLett.19.1264}
     {{\em Phys.\ Rev.\ Lett.}\ {\bf 19} (1967) 1264-1266}.

\bibitem{Salam} A.\ Salam,
  \href{https://dx.doi.org/10.1142/9789812795915_0034}
       {Weak and Electromagnetic Interactions},
in {\em Proc.\ of the 8th Nobel Symposium on ``Elementary
particle theory, relativistic groups and analyticity''},
editor N.\ Svartholm (1968) p.\ 367-377.

\bibitem{Glashow} S.L.\ Glashow,
Partial Symmetries of Weak Interactions,
\href{https://dx.doi.org/10.1016/0029-5582(61)90469-2}
     {{\it Nucl.\ Phys.}\ {\bf 22} (1961) 579-588}.

\bibitem{tHooft} G.\ 't Hooft,
Renormalization of Massless Yang-Mills Fields,
\href{https://dx.doi.org/10.1016/0550-3213(71)90395-6}
     {{\em Nucl.\ Phys.}\ {\bf B33} (1971) 173-199};
Renormalizable Lagrangians for Massive Yang-Mills Fields,
\href{https://dx.doi.org/10.1016/0550-3213(71)90139-8}
     {{\em Nucl.\ Phys.}\ {\bf B35} (1971) 167-188}.\\
G.\ 't Hooft and M.J.G.\ Veltman,
Regularization and Renormalization of Gauge Fields,
\href{https://dx.doi.org/10.1016/0550-3213(72)90279-9}
     {{\em Nucl.\ Phys.}\ {\bf B44} (1972) 189-213}.

\bibitem{BolGiam} C.G.\ Bollini and J.J.\ Giambiagi,
Dimensional Renormalization: The Number of Dimensions
as a Regularizing Parameter,
\href{https://dx.doi.org/10.1007/BF02895558}
     {{\em Nuovo Cim.}\ {\bf B12} (1972) 20-26};
Lowest order divergent graphs in $\nu$-dimensional space,
\href{https://dx.doi.org/10.1016/0370-2693(72)90483-2}
     {{\em Phys.\ Lett.}\ {\bf B40} (1972) 566-568}.

\bibitem{DimReg} W.\ Bietenholz and L.\ Prado, 
40 Years of Calculus in $4 + \varepsilon$ Dimensions,
\href{https://drive.google.com/file/d/1WLNbaCcMLkQkh0bvz6xed4yUTe9YJbSI/view}
     {{\em Bol.\ Soc.\ Mex.\ F\'is.}\ {\bf 26-4} (2012) 227-230}
     \href{https://arxiv.org/pdf/1211.1741}
          {[arXiv:1211.1741 [physics.hist-ph]]};
Revolutionary physics in reactionary Argentina,
\href{https://dx.doi.org/10.1063/PT.3.2277}
     {{\em Physics Today} {\bf 67} (2014) 38-43}.

\bibitem{QCD} H.\ Fritzsch, M.\ Gell-Mann and H.\ Leutwyler,
Advantages of the Color Octet Gluon Picture,
\href{https://dx.doi.org/10.1016/0370-2693(73)90625-4}
     {{\em Phys.\ Lett.}\ {\bf B47} (1973) 365-368}.

\bibitem{Wittig} H.\ Wittig,
Progress on $(g-2)_{\mu}$ from Lattice QCD,
\href{https://arxiv.org/pdf/2306.04165}
     {arXiv:2306.04165 [hep-ph]}.
  
\bibitem{Lederman} L.M.\ Lederman and D.\ Teresi,
``The God Particle'', Dell Publishing, 1993.

\bibitem{Guardian} Interview with Peter Higgs, published in
  \href{https://www.theguardian.com/science/2013/dec/06/peter-higgs-interview-underlying-incompetence}
       {{\em The Guardian}, Dec.\ 6, 2013}.
  
\bibitem{ATLASCMS} ATLAS Collaboration (G.~Aad \textit{et al.}),
Observation of a new particle in the search for the Standard Model
Higgs boson with the ATLAS detector at the LHC,
\href{https://dx.doi.org/10.1016/j.physletb.2012.08.020}
     {{\em Phys.\ Lett.}\ {\bf B716} (2012) 1-29}
[\href{https://arxiv.org/pdf/1207.7214}{arXiv:1207.7214 [hep-ex]}].\\
CMS Collaboration (S.~Chatrchyan \textit{et al.}),
Observation of a new boson at a mass of 125 GeV with the
CMS experiment at the LHC,
\href{https://dx.doi.org/10.1016/j.physletb.2012.08.021}
     {{\em Phys.\ Lett.}\ {\bf B716} (2012) 30-61}
[\href{https://arxiv.org/pdf/1207.7235}{arXiv:1207.7235 [hep-ex]}].

\bibitem{neutrinos} A.\ Aguilar-Ar\'{e}valo and W.\ Bietenholz,
  NEUTRINOS: Mysterious Particles with Fascinating
Features, which led to the Physics Nobel Prize 2015,  
\href{http://www.revistacubanadefisica.org/RCFextradata/OldFiles/2015/Vol32_No2/RCF_32-2_127.pdf}
{{\em Rev.\ Cub.\ F\a'{\i}s.}\ {\bf 32-2} (2015) 127-136}
[more extensive version:
  \href{https://arxiv.org/pdf/1601.04747}
       {arXiv:1601.04747 [physics.pop-ph]]}.

\bibitem{YouTube} \href{https://www.youtube.com/watch?v=m-dNqCbRc\_Y}
  {https://www.youtube.com/watch?v=m-dNqCbRc\_Y}

\bibitem{HiggsBol} D.\ Ayala Garc\'ia and W.\ Bietenholz,
Partícula de Higgs: ¿Qué es, y por qué la necesitamos tanto?,
\href{https://drive.google.com/file/d/1rPwLHnPyK8L-rzK099tzagTh-ankQeNR/view}
     {{\em Bol.\ Soc.\ Mex.\ F\'is.}\ {\bf 26-3} (2012) 161-166}.\\
W.\ Bietenholz,
The Higgs Particle: what is it, and why did it lead to a
Nobel Prize in Physics?,
\href{https://revistacubanadefisica.org/index.php/rcf/article/view/RCF_30-2_109_2013}
     {{\em Rev.\ Cub.\ F\'is.}\ {\bf 30-2} (2013) 109-112}
     \href{https://arxiv.org/pdf/1304.2423}
          {[arXiv:1304.2423 [physics.pop-ph]]}.

\bibitem{WBparti}  W.\ Bietenholz,
What are Elementary Particles? From Dark Energy
to Quantum Field Excitations,
\href{http://www.revistacubanadefisica.org/RCFextradata/OldFiles/2020/v37n2/RCF2020v37p146.pdf}
{{\em Rev.\ Cub.\ F\a'{\i}s.}\ {\bf 37-2} (2020) 146-151}
\href{https://arxiv.org/pdf/2011.07719}
     {[arXiv:2011.07719 [physics.pop-ph]]}.

\bibitem{Shifman} M.\ Shifman (editor), ``Standing Together in Troubled
  Times: Unpublished Letters by Pauli, Einstein, Franck and Others'',
  World Scientific, 2017.

\bibitem{Nambu} Y.\ Nambu,
Axial Vector Current Conservation in Weak Interactions,
\href{https://dx.doi.org/10.1103/PhysRevLett.4.380}
     {{\em Phys.\ Rev.\ Lett.}\ {\bf 4} (1960) 380-382}.\\
Y.\ Nambu and G.\ Jona-Lasinio,
Dynamical Model of Elementary Particles Based on an Analogy
with Superconductivity. I,
\href{https://dx.doi.org/10.1103/PhysRev.122.345}
{{\em Phys.\ Rev.}\ {\bf 122} (1961) 345-358};
Dynamical Model of Elementary Particles Based on an Analogy
with Superconductivity. II,
\href{https://dx.doi.org/10.1103/PhysRev.124.246}
{{\em Phys.\ Rev.}\ {\bf 124} (1961) 246-254}.\\
V.G.\ Vaks and A.I.\ Larkin,
On the Application of the Methods of Superconductivity Theory
to the Problem of the Masses of Elementary Particles,
{\em ZhETF} {\bf 40} (1961) 282-283
[\href{http://jetp.ras.ru/cgi-bin/dn/e_013_01_0192.pdf}
  {{\em JETP} {\bf 13} (1961) 192-193]}.

\bibitem{Goldstone} J.\ Goldstone,
Field Theories with ``Superconductor'' Solutions,
\href{https://dx.doi.org/10.1007/BF02812722}
     {{\em Nuovo Cim.}\ {\bf 19} (1961) 154-164}.
  
\bibitem{GSW} J.\ Goldstone, A.\ Salam and S.\ Weinberg,
Broken Symmetries,
\href{https://dx.doi.org/10.1103/PhysRev.127.965}
     {{\em Phys.\ Rev.}\ {\bf 127} (1962) 965-970}.

\bibitem{Landau} L.D.\ Landau, 
On the angular momentum of a system of two photons,
\href{https://dx.doi.org/10.1016/B978-0-08-010586-4.50070-5}
     {{\em Dokl.\ Akad.\ Nauk.\ SSSR} {\bf 60} (1948) 207-209}.

\bibitem{CERN} \href{https://greybook.cern.ch/country/list}
   {https://greybook.cern.ch/country/list}

\bibitem{Weinberg79} S.\ Weinberg,
Baryon- and lepton-nonconserving processes,
\href{https://dx.doi.org//10.1103/PhysRevLett.43.1566}
{{\em Phys.\ Rev.\ Lett.}\ {\bf 43} (1979) 1566-1570}.

\end{thebibliography}


==> sec1_eng.tex <==
Peter Higgs was born in 1929 in Newcastle, England, spending his
youth partially during World War II, circumstances that somewhat
complicated his schooling. After the war, he studied in London,
first mathematics, then physics. In 1954, only 25 years old,
he completed his Ph.D.\ at King's College.

He then worked temporarily at the University of Edinburgh,
University College, and Imperial College, both
in London. In 1960, he returned to Edinburgh -- a city he loved
and where he had first arrived in 1949, as a hitchhiking student
-- to take up a professorship and stay there for the rest of his life.

In 1964, at the age of 35, he wrote his two famous papers (and
another on the same subject in 1966) \cite{Higgs} that attracted
attention and led to invitations to present seminars at Princeton
and Harvard in 1966. He had to deal with critical audiences;
Sidney Coleman later commented that at Harvard,
``they had been looking forward to tearing apart this idiot who
thought that he could get around
the Goldstone Theorem'' \cite{boson}. It turned out that his concept
stood, but still without phenomenological application (his papers dealt
with a toy model). Additionally, he learned from Yoichiro Nambu
(the referee of one of his papers) about a similar work \cite{EB},
published 15 days before Higgs' first paper on the subject. The
authors were Fran\c{c}ois Englert and Robert Brout, who worked in
Brussels, Belgium. Two months later, yet another related paper
appeared, written in London by Gerald Guralnik, Carl Hagen, and
Tom Kibble \cite{GHK}, but they knew and cited the earlier works
of Englert, Brout, and Higgs.

The mechanism proposed in these three articles was not entirely
new: it had been established in 1962/3 in the context of condensed
matter physics by Philip Anderson \cite{Anderson}. He applied concepts
of Julian Schwinger \cite{Schwinger} for the theoretical explanation
of the mass of a gauge particle to the theory of superconductors.
Englert, Brout, and Higgs presented an extension to relativistic models.

\begin{figure}[h]
    \centering
    \begin{subfigure}{0.3\textwidth}
        \includegraphics[scale=0.8]{higgs_joven.jpeg}
        \caption{}
    \end{subfigure}
    \begin{subfigure}{0.6\textwidth}
        \centering
        \includegraphics[scale=0.25]{brout_englert.png}
        \caption{}
    \end{subfigure}
    \caption{(a) Peter Higgs, who published two brief papers on
    what is now called the Higgs mechanism in 1964, and another
    more extensive one in 1966. (b) Robert Brout (left) and Fran\c{c}ois
    Englert (right). Brout invited Englert to work at Cornell
    University in 1959 for two years as a research associate.
    Afterwards, Brout and Englert moved to the
    University of Brussels, Belgium.}
\end{figure}

\begin{figure}
    \centering
    \begin{subfigure}{0.31\textwidth}
        \includegraphics[scale=2]{hagen.jpg}
    \end{subfigure}	
    \begin{subfigure}{0.31\textwidth}
        \includegraphics[scale=0.5]{guralnik.jpg}
    \end{subfigure}	
    \begin{subfigure}{0.31\textwidth}
        \includegraphics[scale=0.25]{kibble.png}
    \end{subfigure}	
    \caption{Further pioneers of the Higgs mechanism: from
    left to right, Carl Hagen, Gerald Guralnik, and Tom Kibble.} 
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[scale=1]{polyakov_migdal.jpg}	
    \caption{When they were still teenagers, Alexander Migdal (left)
    and Alexander Polyakov (right) discovered the
    Higgs mechanism  independently from the West.}
\end{figure}

\begin{figure}[h]
    \centering
    \begin{subfigure}{0.5\textwidth}
        \centering	
        \includegraphics[scale=0.15]{schwinger.jpg}
    \end{subfigure}\begin{subfigure}{0.5\textwidth}
        \centering	
        \includegraphics[trim = {1cm 1cm 4cm 12cm},clip,scale=0.25]{anderson.jpg}
    \end{subfigure}
    \caption{Left: Julian Schwinger: we can trace back the origin
    of the discovery of
    the Higgs mechanism to his pioneering work on how gauge
    symmetry does not always imply a massless gauge boson.
    Right: Philip Anderson who introduced the mechanism that gives
    mass to gauge bosons in the context of superconductivity.}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[scale=0.3]{higgs_englert_pizarra.jpeg}
    \caption{Peter Higgs and Fran\c{c}ois Englert discussing the
    Lagrangian involving the Higgs field, $\phi$.
    What do you think Higgs is telling Englert? Perhaps he is indicating
    that the fermionic field $\bar \psi_a$ is missing a bar in the
    second line.}
\end{figure}

Independently, in Moscow in 1964, two 19-year-old boys, both named
Alexander (or Sasha), with surnames Migdal and Polyakov, discussed
in great detail what the breaking of a symmetry means \cite{Nobel13}.
They wrote another article, very different but with equivalent
conclusions, which was published in 1966 \cite{MigPol}. In 2010,
Migdal visited Mexico and 
narrated about the difficulties they had in publishing this article,
as the established physics community in the Soviet Union -- under
the leadership of Lev Landau -- rejected the Quantum Field Theory,
which was still very controversial also in the Western world.\footnote{In
Germany, Werner Heisenberg was an influential opponent against
Quantum Field Theory; his preference was the S-matrix formalism.}
Finally, this article got published somewhat late, but even later both
Sashas became famous for other works --- in particular, Polyakov is
known for discovering topological excitations that we now call
{\em instantons.}

The explanation of how gauge particles -- and certain particles
coupled to them -- can have mass soon became known as the \textit{Higgs
mechanism},\footnote{Consulting the original literature does not
lead to a clear explanation of why the terminology excludes
Brout and Englert.}
the subject of Section 2 of this article. Its application to the
phenomenology of elementary particles emerged in 1967/8 by Steven
Weinberg \cite{Weinberg} and Abdus Salam \cite{Salam}. They
incorporated this mechanism into the model of electroweak interaction
that Sheldon Glashow had proposed in 1961 \cite{Glashow} during his
stay in Copenhagen. In fact, Glashow was present at Higgs' seminar
at Harvard, and he appreciated his ``nice model'' \cite{boson}, but
it did not come to his mind that this mechanism could be the remedy
to save his model, which he had already abandoned.

However, this theory -- now known as the {\em electroweak sector of
the Standard Model} -- was still not generally accepted as it was
considered ``non-renormalizable''. In Quantum Field Theories,
divergences almost always appear at high energies, so they
require a ``regularization'', a mathematical manipulation that
turns divergences into finite values. A theory is called
\textit{renormalizable} if, at the end of the calculation, the
regularization can be completely removed and finite predictions
for observables can be obtained (this definition is slightly
simplistic).

The physics community changed its view in 1971/2, thanks to the
work of Gerard 't Hooft, a brilliant PhD student in Utrecht,
Netherlands, who presented evidence in favor of the renormalizability
of this model (partially alongside his advisor, Martin Veltman).
These works \cite{tHooft} were a sensation at that time that caused
a paradigm shift.

\begin{figure}
    \begin{subfigure}{0.5\textwidth}
        \includegraphics[scale=0.5]{weinberg.jpeg}
    \end{subfigure}	
    \begin{subfigure}{0.5\textwidth}
        \includegraphics[scale=0.5]{salam.jpeg}
    \end{subfigure}	
    \caption{Steven Weinberg (left) and Abdus Salam (right)
    independently included the Higgs mechanism into the
    electroweak sector of the Standard Model.}
\end{figure}

\begin{figure}
    \centering
    \begin{subfigure}{0.5\textwidth}
        \centering
        \includegraphics[scale=0.45]{glashow.jpeg}
    \end{subfigure}\begin{subfigure}{0.5\textwidth}
        \centering
        \includegraphics[scale=0.25]{thooft.jpg}
    \end{subfigure}
    \caption{Left: Sheldon Glashow, who invented the original version
    of the electroweak theory. Right: Gerard 't Hooft, famous for
    his work on the renormalization of the Standard Model,
    among other achievements.}
\end{figure}

The key to this milestone was a new method, the \textit{dimensional
regularization}, which is among the main achievements of physics
in Latin America: it was first proposed by two Argentinians, Carlos
Bollini and Juan Jos\'e Giambiagi in 1971, although the publication
\cite{BolGiam} was delayed until 1972. They worked in La Plata, under
difficult circumstances during the military dictatorship \cite{DimReg}.

We add that nowadays less importance is given to the question of
whether or not the Standard Model is renormalizable: the trend is
that it is considered as an effective theory, and its validity in
over a large energy range -- which does not need to extend to infinity
-- is sufficient.

Shortly thereafter, in 1973, the Standard Model of elementary
particles was completely established, with the electroweak sector
\cite{Weinberg,Salam} and another sector of the strong interaction
\cite{QCD}.
The Higgs mechanism is essential to provide masses to a large part
of the elementary particles. This was a revolution in high-energy
physics as we have not seen it anymore in the following half-century;
ever since, progress was relatively slow.

In the 21st century, it is popular to speculate about physics
beyond the Standard Model. However, for now, none of these proposals
have solid support from experimental data. On the other hand,
experiments have confirmed the predictions of the Standard Model
again and again: often it comes out in the news that the Standard
Model has been ``refuted'' by new results, but at the end of the
analysis, and the repetition of the experiments, its predictions
have always triumphed.\footnote{As a recent example, in the latter
part of the last decade, there were news of a tension between the
Standard Model and experiments with the decay of heavy mesons
known as ``B mesons''. In the end, this discrepancy was not
substantiated. The latest hype is the magnetic moment of the
muon, where the experimental value seems slightly different from
the calculation based on the Standard Model. If this is true --
which is far from certain -- the prediction is wrong at the
relative level of $10^{-10}$: if we compare it, for instance,
with the distance between Mexico and Switzerland, about
10,000 km, this corresponds to a possible error of magnitude of
millimeters. But calculations with numerical simulations on the
lattice lead to results closer to the experimental value \cite{Wittig},
a trend that indicates that even this minimal discrepancy could disappear
with a more precise analysis, just like all previously supposed
discrepancies.}

The Standard Model is somewhat incomplete to describe the universe
(in particular gravity, dark matter, and dark energy are missing), but
even so: it is nothing less than the most precise and -- in this
sense -- the most successful theory in the history of science.\\

Higgs no longer participated in this rapid development. He was
already so famous that he could afford to hardly publish research
results anymore from the age of 40.

He was known as a quiet and modest person, almost shy, who did
not seek media attention or to be in the spotlight at events. With
his mindset of abstaining from the show, he can be characterized
as the opposite of Feynman. This characterization corresponds to
the impression of one of the authors (WB) who participated in a
conference in Edinburgh in 1997. Higgs -- who had been emeritus
since 1996 -- appeared at the banquet, but very discreetly, simply
to sit at a table without any spectacle.

This does not mean that Higgs did not have convictions: he was
temporarily an activist for nuclear disarmament and for the
environmental movement as a member of {\em Greenpeace.}\\

Once the Standard Model had been established, its exploration
progressed with intense work in multiple countries.
In the year 2000, all of its particles had already been
experimentally found, except for one: the famous ``Higgs particle'',
involved in the corresponding mechanism, as we will describe
in Section 2.

Again, the nomenclature is perhaps a bit unfair to Englert and
Brout, but this is the convention of the community.
Higgs did not invent this term (this was first done by Ben Lee
\cite{boson}), but he was also uncomfortable with the absurd
nickname ``god particle'' that does not make the slightest sense.
This term was proposed by the editor of a popular science
book \cite{Lederman},
obviously with a commercial objective, but fully irresponsible.
This term became popular and led to endless confusion, for example,
the Catholic Church of Spain believed that the work at CERN had
something to do with theology \cite{Guardian}. We have to
be careful with the terms we use!

In the 21st century, we witnessed an exciting race in the
search for the Higgs particle. In its final phase, it was a
competition between Fermilab (near Chicago) and CERN
(near Geneva, in a bordering region between Switzerland and France).
After initial indications in 2011, in 2012 the Collaborations
ATLAS and CMS, both working independently
at the Large Hadron Collider (LHC) at CERN, presented
indirect but compelling evidence for the observation of the
so wanted Higgs particle \cite{ATLASCMS}.

\begin{figure}

\begin{subfigure}{0.5\textwidth}
	\includegraphics[scale=0.27]{atlas.jpg}
\end{subfigure}	
\begin{subfigure}{0.5\textwidth}
	\includegraphics[scale=0.9]{cms.jpeg}
\end{subfigure}	
\caption{Detectors of the Collaborations ATLAS (left) and CMS
(right) at CERN that confirmed the existence of
the Higgs boson of the Standard Model.
Both are multipurpose detectors, used to
analyze collisions between particles of very high energy.}
\end{figure}

With this, the entire set of particles of the Standard Model
was observed. Thus it was confirmed that the Higgs mechanism
is realized in nature, 48 years after its theoretical proposal.
This took almost twice as long as the observation of the neutrino
(predicted by Wolfgang Pauli in 1930, and detected by Clyde Cowan,
Frederick Reines and collaborators in 1956),\footnote{Ref.\
\cite{neutrinos} reviews the history and properties of neutrinos,
from a semi-popular perspective.}
we see that sometimes it is worth being patient.

In particular, it was worth it for Englert and Higgs, who received
the Nobel Prize in 2013 for their correct prediction \cite{Nobel13};
sadly, Brout had died shortly before, in 2011.
In April 2024, we received news of Higgs' passing away,
at the age of 94, after a brief illness.

\begin{figure}
\centering
\includegraphics[scale=.3]{higgs_englert2.jpeg}
\caption{On July 4, 2012, CERN publicly announced the
discovery of the Higgs boson. Peter Higgs, moved to
tears at the ceremony, said \cite{YouTube}: ``... congratulations
to everybody involved in this tremendous achievement. For me it
is really an incredible thing that this happened in my lifetime''.
The Royal Swedish Academy of Sciences awarded the Nobel Prize
in Physics in 2013 to Fran\c{c}ois Englert (left) and Peter
Higgs (right) for ``the theoretical discovery of a mechanism
that contributes to our understanding of the origin of mass
of subatomic particles $\dots$''.}
\end{figure}


==> sec2_eng.tex <==
To the best of our knowledge, the world consists of
{\em elementary particles,}
which are indivisible, and occur in a few types (say 25, but
it depends a bit on how one counts). Famous examples are the
electron and the photon (the particle of light).

Their relativistic description is based on ``fields'', abstract
quantities, present throughout the universe, at any time. At some
space-point, a field can take different states, depending on time.
If the fields in a region are in their ground states, we perceive
the vacuum. Excitations are quantized and manifest as elementary
particles; this is the idea of the \textit{Quantum Field Theory}.

There is a field for each type of elementary particle, and their
excitations can move (like waves), interact, generate, and destroy
particles (this is a requirement for compatibility with Special
Relativity, which is lacking in Quantum
Mechanics).\footnote{Ref.\ \cite{WBparti} presents a more
extensive popular science description of elementary particles.}

A central concept is {\em symmetry:} symmetry means the invariance
of physical properties under a group of transformations of one or
more fields. We distinguish between {\em global} and {\em local}
symmetries:

\begin{itemize}

\item If a symmetry is {\em global}, a field transforms in the same
way everywhere. One can imagine a group of people doing collective
gymnastics, all making the same movement, which could be synchronized
with music.
(The image is a bit simplistic because the fields transform in
the same way even throughout space-time.)
  
\item The case of a {\em local} symmetry can be imagined as chaotic
gymnastics: each person moves as he/she wishes, independently. This
means that the fields can be transformed independently at each point
in space-time.

It is clear that this type of symmetry allows many more transformations.
Achieving local symmetry is far more difficult but leads to stronger
restrictions, and therefore to a powerful ability to make predictions.
  
Technically, an additional field is introduced, known as the
{\em gauge field,} which transforms in such a way as to compensate for
the relative change between nearby points in a simultaneous
transformation. This successful concept describes the transmission
of interactions, but it only works if local symmetry is exact.
  
\end{itemize}

An important category of particles is known as ``fermions'':
the (known) elementary fermions have spin $1/2$ in natural
units.\footnote{To use natural units, one sets Planck's constant
and the speed of light in vacuum to 1, $\hbar = c = 1$.}
Spin is an internal degree of freedom that manifests like an angular
momentum. The fermions of the Standard Model are the electron,
its two heavier ``cousins'' (the muon and the tauon), neutrinos
(much lighter and electrically neutral)\footnote{The set of
the electron, muon, tauon, and the three neutrinos is known as
the {\em leptons}.}
and quarks (constituents of composite particles, such as the
proton and the neutron).

A fermion can exist in two variants, with ``chirality'' left
or right; it can be imagined as hands,\footnote{Indeed, the
term comes from ``kheir'', which means ``hand'' in Greek.}
or gloves, which are left or right, but for fermions
in an abstract sense.

Suppose {\it e.g.}\ an electron without mass: in this case,
the left ($e_L$) and right ($e_R$) electron are independent,
and their spin points against (for $e_L$) or in (for $e_R$)
their direction of motion (a particle without mass cannot be
at rest). This is symbolically illustrated in Figure \ref{electron}.

\begin{figure}
\centering
\includegraphics[scale=1]{chiral.pdf}
\caption{Symbolic illustration of a massless electron with
left-handed chirality, $e_L$, and right-handed chirality, $e_R$.
The direction of motion is indicated by the thin arrow, and
the direction of spin by the bold arrow. For left-handed chirality,
the velocity and spin point in opposite directions, whereas
for right-handed chirality, they point in the same direction.}
\label{electron}
\end{figure}

Including a mass term requires a product of the fields of the
left and right electrons (one can imagine the two hands holding
onto each other). Then they are no longer independent, and under
symmetry they have to transform in the same way.

This is, however, not the case in Glashow's electroweak theory
\cite{Glashow}: this theory allows, for example, local (``gauge'')
transformations that only affect $e_L$, but not $e_R$.
Here was the problem: this theory seemed to be incompatible
with the mass term of the electron (and other fermions), but we
know that the electron does have a mass of
$M_e \simeq 0.511\ {\rm MeV}$ (still in natural units).

In fact, the situation was even worse. The gauge particles that
transmit weak force are called $W^{\pm}$, $Z^0$ (with electric
charge $\pm1, \, 0$), for example, the $W$ are responsible for
radioactive decay. This force has a very short range (about
$10^{-17}$~m) that can only be explained if $W^{\pm}$, $Z^0$ have
large masses (they are among the heaviest elementary particles
we know, with masses of $M_W = 80.4 \, {\rm GeV}$ and
$M_Z = 91.2\,{\rm GeV}$). But just like the mass of the electron,
it seems that gauge symmetry, which has to be exact, requires
$m_W = m_Z = 0$.

The puzzle of where the masses of gauge particles could possibly
come from was a ``killer question'' with which Wolfgang Pauli ruined
a seminar by Chen-Ning Yang in Princeton in 1953 on gauge
theories with a non-Abelian symmetry group (now known as
Yang-Mills theories). Without knowing the Higgs mechanism,
Yang could not answer, but Pauli insisted so much that Yang
sat down, frustrated. Finally, Robert Oppenheimer had to encourage
him to continue his talk \cite{Shifman}.

So, how does the salvation of this theory, the Higgs mechanism,
work? First, another field is added, the {\em Higgs field}, we
use the notation $\phi (x)$.
The variable $x$ is a point in space-time, and $\phi$ is a
scalar field, its fluctuations represent particles with spin 0.
To establish an electron mass term, now a product of {\em three}
fields is formed, $e_L$, $\phi$, and $e_R$.\footnote{We actually
need partially anti-fields, which represent anti-particles, but
we ignore this aspect in the context of this popular science article.}
The Higgs field also transforms under local symmetry, in such a
manner that the term as a whole is gauge invariant.

So in this way, a permissible term (gauge invariant) can be added,
but does this provide mass to the electron?
Possibly yes, it can work with the following scenario.

At low energies, the Higgs field ``freezes'' to its ground state,
manifesting almost as a constant. This constant does not have to
be zero: indeed, $\phi$ has 4 real components, but we can imagine
there to be only 2, $\phi_1 , \, \phi_2 \in \mathbb{R}$, parameterizing
a plane. This field comes with a potential $V(\phi_1, \phi_2)$ shaped
like a Mexican hat, with zero value at the center, but there is a ring of
minima corresponding to a value $|\phi|^2 = \phi_1^2 + \phi_2^2 > 0$,
as illustrated in Figure \ref{sombrero}. This ``vacuum expectation
value'' takes on the role of the electron's mass that the model needs
(up to a coefficient), $M_e \propto |\phi|$, and similarly, the
masses $M_W$ and $M_Z$ are obtained, all in agreement with gauge
symmetry (we will return to this point).

It seems  all fine, but there is still another problem, and this
is the point that Coleman referred to in his comment on Higgs'
seminar at Harvard, which we quoted in Section 1.
The Mexican hat potential has a symmetry under rotations about the
central axis. We assume the field $\phi$ to choose one of the minima:
the process of this choice is denoted as ``spontaneous symmetry
breaking'': from the perspective of a specific minimum, the
rotation symmetry is no longer apparent. In Ref.\ \cite{HiggsBol},
we described this process with the analogy of the \textit{Buridan's
Donkey}, which is thirsty and surrounded by a water trough but has
to decide which direction to walk in order to drink water.

Small fluctuations of the field beyond its minimum state correspond
to particles. If a fluctuation is \textit{radial}, it costs energy
because the potential rises -- this is a massive particle (the
curvature of the potential in the radial direction corresponds
to its mass squared). On the other hand, a \textit{tangential}
fluctuation does not require any energy, as the field stays at its
energy minimum. This is an example of a massless particle, known
as a \textit{Nambu-Goldstone boson} \cite{Nambu,Goldstone}.
According to the Goldstone Theorem \cite{GSW}, these bosons appear
when a continuous symmetry (such as rotation in this example)
is spontaneously broken.

If the mechanism works as described above, the question remains:
where is this Nambu-Goldstone boson? Being massless, it should
play a relevant role and dominate physics at low energies
(where very heavy particles are not visible). But no particle
of this kind has been observed. So, to justify the mechanism,
one has to ``get around the Goldstone Theorem'', as Coleman put it,
but the physicists at Harvard doubted whether this was possible.
They were not alone; for example, Klaus Hepp, a prominent
mathematical physicist, warned Higgs that this might not work
because the Theorem was proven using C$^{*}$ algebra, a formalism
that Higgs was not familiar with, but he expressed doubts about
the assumptions in this proof \cite{boson}.

We now know that the Theorem is indeed correct, but it only refers
to the breaking of a \textit{global} continuous symmetry -- this
assumption was hidden. The crucial observation was that the
situation is different in the case of a \textit{local} symmetry:
in this case, the minima are connected by local transformations,
or gauge transformations, thus they are physically identical. So there
are no physical fluctuations between the minima, and there are
no Nambu-Goldstone bosons. What happens -- and this completes the
Higgs mechanism -- is that the gauge boson acquires mass, meaning
that the degree of freedom of the Nambu-Goldstone boson turns into
the longitudinal degree of freedom of the gauge boson (without mass,
it only has transverse degrees of freedom). In popular language,
it is said that the gauge boson {\em ``eats up''} the Nambu-Goldstone
boson: the latter is no longer there, but the former becomes ``fat''.

This had been observed by Anderson before in a typical superconductor:
inside it, at very low temperature, the photon acquires mass, hence
it can hardly penetrate the superconductor -- a phenomenon known
as the \textit{Meissner-Ochsenfeld effect}. Brout, Englert, and
Higgs extended this effect to relativistic models \cite{EB,Higgs},
and Weinberg and Salam to the phenomenology of electroweak
interaction \cite{Weinberg,Salam}. We mentioned that the Higgs
field has 4 real components: there is always one massive radial
fluctuation, and thus 3 Nambu-Goldstone bosons if we are dealing with
a global symmetry. When it is promoted to a local symmetry, the bosons
$W^+$, $W^-$, and $Z^0$ ``eat up'' these Nambu-Goldstone bosons
and acquire masses, while the photon remains massless (under
normal circumstances) and describes long-range electromagnetism.

\begin{figure}
    \centering
    \includegraphics[scale=2]{higgspotential_eng.pdf}
    \caption{The Higgs potential: from the top perspective, the
    potential is rotationally symmetric. However, from the
    perspective of the ball, the potential seems not to exhibit
    this symmetry, which is ``spontaneous broken''.
    Tangential fluctuations of the field along the circle of minima
    manifest as a Nambu-Goldstone boson if the symmetry is global.
    If the symmetry is local, this Nambu-Goldstone boson is
    ``eaten of'' by a gauge field that acquires mass. Radial
    fluctuations, perpendicular to the circle of minima, manifest
    as a massive particle. If dealing with the Higgs potential as in
    the Standard Model, this massive particle is the famous Higgs
    boson.}
    \label{sombrero}
\end{figure}

We have seen that the mechanism also provides a mass to the electron,
and it similarly applies to the muon, tauon, and all the quarks.
And what about the Higgs field? We know that 3 of its 4 components
would be Nambu-Goldstone bosons that disappear, but the fourth
component remains, corresponding to the radial fluctuation, {\it i.e.},
to a massive particle. Its existence is a prediction of the Higgs
mechanism, and in this respect, the second article by Higgs from
1964 was somewhat more explicit than the other original works.
This was still in the context of toy models, but once applied to
a phenomenological model, one concluded that such a
\textit{Higgs particle} has to be \textit{observable}.

The theory does not predict the mass of the Higgs particle,
$M_{\rm H}$ (only bounds could be derived, which were a topic
of discussion over many years), so its experimental search was
challenging. At the beginning of the 21st century, the experiments
of the Large Electron-Positron Collider (LEP) at CERN showed
that it must have a mass $M_{\rm H} > 114\, {\rm GeV}$. So it was
known to be very heavy (if it exists), requiring high-energy
collisions for its creation. This also implies that its lifetime
is very short, decaying on average in $10^{-22}$ seconds, so it
cannot leave traces in any detector.

An experiment has to capture the products of its decay that
allow the reconstruction of the Higgs particle as an intermediate
state, or ``resonance'' -- for a very short time -- in a high-energy
collision. The analysis of the particles resulting at the end of
the process enables the reconstruction of the Higgs particle properties,
in particular its mass of $M_{\rm H} \simeq 125\, {\rm GeV}$
and its spin 0, confirming it to be a scalar particle.

In the cleanest channel observed, the decay of the Higgs particle
ends with two photons, a final state that would not be possible if,
for example, the original particle had spin 1, as Landau had
proved \cite{Landau}. But the ATLAS and CMS experiments studied
(independently) many more decays in great detail -- such as,
for instance, with a final state of four leptons -- leaving
no doubt about the existence of the Higgs particle, and the
corresponding mechanism.

\begin{figure}
    \centering
    \includegraphics[scale=0.2]{atlas-higgs.jpg}
    \caption{Possible decay channels of the Higgs boson when
    decaying into two $Z$ bosons, each of which decays into a
    lepton-antilepton pair. In this picture, we observe two
    such pairs (red and blue lines) that might have been
    produced by the decay of a Higgs boson.}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[scale=0.42]{lhc.jpg}
    \caption{The Large Hadron Collider (LHC) is located on the
    border region between France and Switzerland. Its four main
    experiments are called ATLAS and CMS (which independently
    found evidence of the existence of the Higgs boson), ALICE,
    and LHCb.
    The following Latin American countries are involved in
    these collaborations \cite{CERN}: Argentina, Brazil, Chile,
    Colombia, Costa Rica, Cuba, Ecuador, Mexico, Peru.}
\end{figure}

This represents a spectacular success of elementary particle
physics. Nevertheless, not everything is resolved yet. From a
conceptual perspective, the \textit{hierarchy problem} remains,
and regarding phenomenology, the Higgs mechanism does not explain
the origin of all masses we observe. We end with brief comments
on these issues:

\begin{itemize}

\item \textit{Hierarchy problem:} If we start with a classical
system (without quantum effects) and assume a mass $m_{\rm H}^{(0)}$
on the order of masses of other particles, it is natural
that quantum corrections drastically increase this mass to
a value $m_{\rm H}$ on the order of the ``Planck scale''
(determined by the gravitational constant). But this leads to
a huge mass $m_{\rm H}$, typically about $10^{17}$ times
its observed value.

One could assume an extremely negative value of $m_{\rm H}^{(0)}$,
so that the quantum effect is almost entirely canceled out,
leaving a tiny remainder of 125 GeV. But this approach
-- with a cancellation between two tremendous contributions
leaving a tiny remainder -- does not seem natural. This is
known as the ``hierarchy problem''. However, it is not a
paradox, one can consistently arrive at 125 GeV, and the question
of how severe this problem is, is somewhat philosophical.
The extent of the hierarchy gap also depends on the regularization
that one applies.

\item {\em Neutrinos} (denoted by $\nu$) play a special role:
the traditional form of the Standard Model assumed
them to have mass zero, $M_{\nu} =0$, and only the
left-handed neutrino, $\nu_L$, to exist.

This is consistent in theory, but at the end of the 20th
century, it was observed that neutrinos do have a small mass,
$m_{\nu}>0$ -- we reiterate that Ref.\ \cite{neutrinos}
provides a semi-popular review of the topic.

At first sight, according to our previous description, it
seems inevitable that the right-handed neutrino, $\nu_R$, exists.
This allows the application of the Higgs mechanism to neutrinos,
and also another type of mass, only for the $\nu_R$, known as
``Majorana mass''.

However, the $\nu_R$ is not observed, and its existence is not
truly inevitable: we can construct a mass term involving only
the $\nu_L$ field \cite{Weinberg79}.
This term is non-renormalizable, but we
mentioned in Section 1 that the importance given to of this property
is diminished. So this scenario would be the alternative, within
the framework of the Standard Model interpreted as an effective
theory that works in a certain energy range.

\item Up to this point, the Higgs mechanism explains the masses
of elementary particles (with the possible exception of neutrinos),
and there are other particles like the photon that remain massless.
It seems like a complete picture of the origin of mass.

However, the real world is different: in reality, the mass of
a macroscopic object in our everyday life originates only to
$1 \dots 2 \, \%$ from the Higgs mechanism, which leads to the
masses of quarks.

These everyday masses consist mainly of nucleon masses
(protons and neutrons), which essentially consist of energy
from \textit{gluons} (other gauge particles, which transmit
the strong interaction): they have zero mass, but are confined
inside a nucleon (or another particle composed by the strong
interaction). Their energy manifests as almost the entire mass
of the nucleon, while the masses of quarks only provide
the aforementioned contribution of $\sim 1 \dots 2 \, \%$.

The interior of a nucleon is a very, very complex system,
for a long time it seemed impossible to calculate anything
conclusive about it. However, a little over a decade ago, it
became possible to compute, for example, the mass of the nucleon,
$M_N \simeq 939\,{\rm MeV}$, from first principles, up to an
uncertainty of the order of 1\,\%. This calculation captures the
hyper-complicated mess of gluons (and ``sea quarks'', unstable
pairs of a quark and its anti-quark), and the result is compatible
with experiments. The question of how these calculations are possible
would be a topic for another article $\dots$

\end{itemize}

